Reward-Biased Maximum Likelihood Estimation for Linear Stochastic Bandits

Modifying the reward-biased maximum likelihood method originally proposed in the adaptive control literature, we propose novel learning algorithms to handle the explore-exploit trade-off in linear bandits problems as well as generalized linear bandits problems. We develop novel index policies that we prove achieve order-optimality, and show that they achieve empirical performance competitive with the state-of-the-art benchmark methods in extensive experiments. The new policies achieve this with low computation time per pull for linear bandits, and thereby resulting in both favorable regret as well as computational efficiency.

==> 1-intro-reward.tex <==
\section{Introduction}
\label{section:intro}

% Overview of BMLE
% Main argument:
% 0. Overview of adaptive control and Identifiability issue
{\color{red}I am still working on this ...} 
The problem of decision making for an initially unknown stochastic system, called {\color{blue} stochastic adaptive control \cite{kumar1986stochastic}}, was examined in the control theory community beginning in the 1950s. It was recognized early on by \citet{feldbaum1960dual1,feldbaum1960dual2} that control played a dual role, that of exciting a system to learn its dynamics, as well as satisfactorily regulating its behavior, therefore dubbed as the problem of ``dual control.''
This leads to a central problem of identifiability: As the controller begins to converge, it ceases to learn about the behavior of the system to other control actions. This issue was quantified by \citet{borkar1979adaptive} within the setting of adaptive control of Markov chains. Consider a stochastic system with a state-space $X$, control or action set $U$, modelled as a controlled Markov chain with transition probabilities $\mbox{Prob}(x(t+1)=j \vert x(t)=i, u(t)=u) = p(i,j;u,\theta_*)$ dependent on an unknown parameter $\theta_*$ lying in a known set $\Theta$, where $x(t)$ is the state of the system at time step $t$, and $u(t)$ is the action taken at that time. Given a \pch{one-step reward function $r(i,u)$}, let $\phi: X \times \Theta \rightarrow U$ denote the optimal stationary control law as a function of $\theta \in \Theta$ for the \pch{long-term average reward problem: $\max \frac{1}{T} \sum_{t=0}^{T-1} r(x(t),u(t))$}, i.e., $u(t)=\phi(x(t),\theta)$ is the optimal action to take if the true parameter is $\theta$.
Since $\theta_*$ is unknown, consider a ``certainty-equivalent'' approach: At each time step $t$, let $\widehat{\theta}_{\text{ML}}(t) \in \argmax_{\theta \in \Theta} \sum_{s=0}^{t-1} \log p(x(s),x(s+1),u(s),\theta)$ denote the Maximum Likelihood (ML) estimate of $\theta_*$, with ties broken according to any fixed priority order. Then apply the action $u(t)=\phi(x(t), \widehat{\theta}_{\text{ML}}(t))$ appropriate to that estimate.
{\color{blue}It was shown in \cite{}} that under an irreducibility assumption, the parameter estimates $\widehat{\theta}_{\text{ML}}(t)$ converge to a random limit $\check{\theta}$ satisfying \begin{equation}
p(i,j,\phi(i, \check{\theta}),\check{\theta}) = p(i,j,\phi(i, \check{\theta}),\theta_*) \quad \quad  \forall i,j \in X. \label{eq closed-loop identification}
\end{equation}
That is, the closed-loop transition probabilities under the control law
$\phi(\cdot, \check{\theta})$ are correctly
determined. However, the resulting long-term average \pch{reward} 
is not optimal for $\theta_*$ since $\phi(\cdot,\check{\theta})$ need not be optimal for the true parameter $\theta_*$.

A key observation concerning the result
(\ref{eq closed-loop identification})
was made by Kumar and Becker in \cite{kumar1982new}. Denote by $J(\phi, \theta)$ the long-term average \pch{reward} incurred when the stationary control law $\phi$ is used if the true parameter is $\theta$, and by \pch{$J(\theta) := \max_\phi J(\phi, \theta)$} the optimal long-term average \pch{reward} attainable when the parameter is $\theta$.
Then,
\pch{
\begin{equation}
J(\check{\theta}) \overset{(a)}{=} J(\phi(\cdot,\check{\theta}), \check{\theta}) \overset{(b)}{=} J(\phi(\cdot,\check{\theta}), \theta_*) \overset{(c)}{\leq} J(\theta_*). \label{eq cost inequality}
\end{equation}
}
where the key equality $(b)$ that the \pch{rewards} under $\phi(\cdot, \check{\theta})$ are the same under the parameters $\check{\theta}$ and $\theta_*$ follows from the closed-loop identification property
(\ref{eq closed-loop identification}), while $(a)$ holds trivially since $\phi(\cdot,\check{\theta})$ is optimal for $\check{\theta}$, and $(c)$ also holds trivially
since
$\phi(\cdot,\check{\theta})$ is not necessarily optimal for $\theta_*$.
Therefore one makes the key observation that
the limiting parameter estimate $\check{\theta}$ is biased in favor of parameters with \pch{\emph{smaller} reward}. 
Exploiting this observation, \cite{kumar1982new} proposed delicately biasing the ML parameter estimation criterion in the reverse way in favor of parameters with \pch{\emph{larger} reward}, and suggested using the resulting \pch{\emph{biased ML estimate} (BMLE) $\widehat{\theta}_{\text{BMLE}}$}:
\begin{equation}
\widehat{\theta}_{\text{CBMLE}}(t) \in {\argmax}_{\theta \in \Theta} \{-\alpha(t) J(\theta)+ \sum_{s=0}^{t-1} \log p(x(s),x(s+1),u(s),\theta) \},
\end{equation}
where $\alpha(t)>0$ with $\alpha(t) \to + \infty$, 
but small in that $\frac{\alpha(t)}{t} \to 0$.
This delicate modification still preserves the good properties of the ML estimate for any ``frequent'' limit point $\check{\theta}$, (i.e., which occurs as a limit along a sequence with sufficient density in the integers),and therefore retains the property (\ref{eq closed-loop identification}). Hence
(\ref{eq cost inequality}) also continues to hold.
However, since $\alpha(t) \to +\infty$ the limit $\check{\theta}$ satisfies
\begin{equation}
J(\check{\theta}) \leq J(\theta_*). \label{eq reverse inequality}
\end{equation}
From (\ref{eq reverse inequality}) and (\ref{eq cost inequality}) it follows that $J(\phi(,\cdot,\check{\theta}),\theta_*) = J(\theta_*)$,
i.e., $\phi(\cdot, \check{\theta})$ is optimal for the unknown $\theta_*$.

The CBMLE methods holds potential as a general purpose method for learning of dynamic systems. 
However, its analysis was confined to long-term average optimality, which only
assures that the regret is $o(t)$ . 
While being a theoretically well-grounded approach in terms of asymptotic behavior, it has remained largely unknown whether the BMLE principle can attain superior finite-time performance.
Motivated by this, there has been recent interest in revisiting the \pch{BMLE} method to explore its potential for contemporary problems. Recently, its regret performance has been established
for classical multi-armed bandits for the exponential family of measures \cite{liu2019bandit}. However, classical bandits do not allow the incorporation of ``context,'' which is important in several applications \cite{li2010contextual,lu2010contextual,chapelle2011empirical,li2016collaborative,tewari2017ads}. In this paper we examine the performance of the \pch{BMLE} method both for linear contextual bandits as well nonlinear. 
Linear contextual bandits and its variants have been popular models for abstracting the sequential decision making in various applications, such as recommender systems \cite{li2010contextual} and mobile health \cite{tewari2017ads}.
In this paper, our goal is to study the finite-time regret performance of the BMLE algorithm for standard linear bandits {\color{black}as well as the generalized linear ones}. 
To achieve this, we adapt the BMLE principle to linear contextual bandits by taking the following steps: (i) We first propose a specific type of reward-bias term. 
\pch{An important innovation that we have found necessary is
to introduce a regularization term into the reward-biased maximum likelihood criterion. }
(ii) Another innovation we introduce is to use a Gaussian likelihood function even
when the distribution of the noise is unknown.
The usage of the Gaussian distribution as a pseudo-likelihood allows us to derive simple closed-form indices.
(iii) Despite the use of a pseudo-likelihood, we show that the BMLE index derived from the Gaussian likelihood attains an order-optimal regret bound for the general, possibly non-parametric, sub-Gaussian rewards.
(iv) Based on the results for the linear bandits, we extend the techniques to the generalized linear models and show that the same regret bound can still be attained in the general case.
(v) We show that the resulting \pch{BMLE}-based {\color{blue}generalized linear bandits} have a cumulative regret of the order of $\sqrt{T} \log T$. {\color{blue}This shaves a factor of $\sqrt{\log T}$ from \cite{filippi2010parametric}}, and achieves the same regret bound as that of UCB-GLM in \cite{li2017provably}.
We also conduct large-scale experiments to demonstrate the effectiveness, efficiency and scalability of the proposed algorithms.
% TODO: One more sentence for describing linear bandits


% In the 
% From this \ref{eq cost inequality}
% The ``bet on the best'' principle \cite{kumar1982new,bittanti2006adaptive} has been a well-known approach to achieving asymptotic optimality for adaptive control problems, where the dynamic behavior of a stochastic system is determined by an unknown parameter $\theta$ that belongs to some parameter set $\Theta$.
% % Explain adaptive control
% In the adaptive control formulation \cite{kumar2015stochastic}, the goal is to sequentially apply actions in order to minimize the long-term average cost without the knowledge of the true system parameters. 
% To learn a self-optimizing strategy, the learning process is usually decoupled into two major stages: \textit{inference} and \textit{control}.
% %For inference, certainty equivalence 
% As an illustrative example, consider a controlled Markov chain with finite states and actions. 
% In this example, the unknown parameter $\theta$ corresponds to the transition probabilities, and the set $\Theta$ includes all feasible transition probability matrices.
% In the inference phase, at each decision time $t$, the unknown parameter $\theta$ can be estimated by maximum likelihood estimator $\hat{\theta}_t^{\text{MLE}}$ given the observed history $\mathcal{H}_t$.
% %Given the observed history, the unknown parameter $\phi$ can be estimated through maximum likelihood estimation. 
% Such estimation scheme is also known as the \textit{certainty equivalence} principle.
% In the control phase, after observing the system state $s_t$, the controller follows some stationary control law $\phi$ and applies an action $\phi(s_t;\hat{\theta}^{\text{MLE}})$, which would be optimal if $\theta^{\text{MLE}}$ is the true system parameter.
% Despite the simplicity and wide applicability of the certainty equivalent design, it is known to suffer from the \textit{closed-loop identifiability} issue and is sub-optimal \cite{kumar2015stochastic,mandl1974estimation,borkar1979adaptive}.
% %This issue arises from that the selected actions need to serve for dual purposes, i.e. identification and control, it may fall short to the \textit{closed-loop identifiability} issue \cite{kumar2015stochastic,mandl1974estimation,borkar1979adaptive}, where 
% %However, the certainty equivalence principle is known to suffer from the close-loop identifiability issue.

% To address this fundamental issue, the ``bet on the best'' principle estimates the parameter $\theta$ by resorting to the \textit{cost-biased} maximum likelihood estimation (BMLE), in which an additional cost-dependent term is augmented to the MLE.
% Specifically, the estimator of $\theta$ under BMLE is given by 
% \begin{equation}
%     \hat{\theta}^{\text{BMLE}}_t:=\argmax_{\theta\in \Theta} \hspace{3pt}\{\ell(\mathcal{H}_t;\theta)-\alpha(t) \cdot \log(J(\theta))\},
% \end{equation}
% where $\ell(\mathcal{H}_t;\theta)$ denotes the log-likelihood of the observed history $\mathcal{H}_t$ under $\theta$, $J(\theta)$ denotes the optimal long-term average cost under $\theta$, and $\alpha(t)$ is a sub-linear positive-valued function that satisfies two conditions: (i) $\lim_{t\rightarrow \infty}\alpha(t)=\infty$, and (ii) $\lim_{t\rightarrow \infty}\alpha(t)/t=0$.
% These requirements for $\alpha(t)$ manifest the design principles of BMLE: 
% \begin{itemize}
%     \item By the condition (i), the cost-bias term aims to provide sufficient exploration towards the cost-minimizing parameters (as suggested by the name "bet on the best").
%     \item The condition (ii) suggests that the guided exploration resulting from the cost-bias term would diminish as the system evolves indefinitely.
% \end{itemize}
% Under a properly-chosen bias term $\alpha(t)$, the BMLE algorithm has been shown to achieve long-term average optimality for various stochastic systems \cite{kumar1982new}.
% While being a theoretically well-grounded approach in terms of asymptotic behavior, it remain largely unknown whether the BMLE principle can attain superior finite-time performance.
%Despite the asymptotic optimality, it remains unclear whether the BMLE principle can achieve good finite-time performance. 
% Explain close-loop identifiability

% 1. Overview of Generalized linear bandit

% 2. Cast as an adaptive control problem
% 3. 
% 4. BMLE

% In this paper, our goal is to study the finite-time regret performance of the BMLE algorithm for linear contextual bandits. 
% Linear contextual bandits and its variants have been popular models of abstracting the sequential decision making in various applications, such as recommender systems \cite{li2010contextual} and medical treatment.
% % TODO: One more sentence for describing linear bandits
% When put in the context of adaptive control, bandit learning for linear models can be addressed by alternating between the inference phase and the control phase.
% To achieve this, we adapt the BMLE principle to linear contextual bandits by taking the following steps: (i) We first propose a specific type of reward-bias term; 
% (ii) To derive simple closed-form indices, we further propose to use the Gaussian distribution as the pseudo likelihood required by the BMLE procedure. 
% Despite the use of pseudo likelihood, we show that the BMLE index derived from the Gaussian likelihood attains an order-optimal regret bound for the general, possibly non-parametric, sub-Gaussian rewards.
% Based on the results for the linear bandits, we extend the techniques to the generalized linear models and show that the same regret bound can still be attained in the general case.
%From the perspective of adaptive control, the stochastic multi-armed bandit problems can be cast as adaptive control problems.
%In this paper, we focus on a broad class of contextual bandit models, namely the generalized linear bandits.


%One popular approach is to utilize a bias in the maximum likelihood estimation.
%This approach originated from the work \cite{kumar1982new}.
%The ``bet on the best'' principle, which was first coined by Campi \cite{bittanti2006adaptive}, has been a widely-used approach to learning with unknown Markov decision processes.

% Connection between BMLE and OFU: Benefits


% Summary of main technical contents


%  Main contributions
%The main contributions of this paper can be summarized as follows:
%\begin{itemize}
%    \item We propose a new index-type algorithm for linear bandits by leveraging the BMLE principle. Specifically, we propose to first utilize the parametric distributions to derive a simple index for each arm.
%    \item The proposed algorithm is shown to achieve order-optimal regret for the general sub-Gaussian rewards.
%\end{itemize}
